Distributed Multi-Agent Bandits Over Erd\H{o}s-R\'enyi Random Networks

We study the distributed multi-agent multi-armed bandit problem with heterogeneous rewards over random communication graphs. Uniquely, at each time step $t$ agents communicate over a time-varying random graph $G_t$ generated by applying the Erd\H{o}s-R\'enyi model to a fixed connected base graph $G$ (for classical Erd\H{o}s-R\'enyi graphs, $G$ is a complete graph), where each potential edge in $G$ is randomly and independently present with the link probability $p$. Notably, the resulting random graph is not necessarily connected at each time step. Each agent's arm rewards follow time-invariant distributions, and the reward distribution for the same arm may differ across agents. The goal is to minimize the cumulative expected regret relative to the global mean reward of each arm, defined as the average of that arm's mean rewards across all agents. To this end, we propose a fully distributed algorithm that integrates the arm elimination strategy with the random gossip algorithm. We theoretically show that the regret upper bound is of order $\log T$ and is highly interpretable, where $T$ is the time horizon. It includes the optimal centralized regret $O\left(\sum_{k: \Delta_k>0} \frac{\log T}{\Delta_k}\right)$ and an additional term $O\left(\frac{N^2 \log T}{p \lambda_{N-1}(Lap(G))} + \frac{KN^2 \log T}{p}\right)$ where $N$ and $K$ denote the total number of agents and arms, respectively. This term reflects the impact of $G$'s algebraic connectivity $\lambda_{N-1}(Lap(G))$ and the link probability $p$, and thus highlights a fundamental trade-off between communication efficiency and regret. As a by-product, we show a nearly optimal regret lower bound. Finally, our numerical experiments not only show the superiority of our algorithm over existing benchmarks, but also validate the theoretical regret scaling with problem complexity.

==> new_neurips_2025/secs/application.tex <==
\section{Applications on Variant Graphs}

\begin{assumption}[Time-invariant graph]
\label{ass: fixed_g}
    Assume $\mathcal{G}$ is any undirected connected graph. The communication network of the multi-agent system is described by a time-invariant graph $G = \mathcal{G}$. 
\end{assumption}


\begin{assumption}[Classical Erdős–Rényi random graph]
\label{ass: c_er_g}
    Assume $\mathcal{G}$ is a complete graph. The communication network of the multi-agent system at time $t$ is modeled by a random graph $G_t$, which is generated over the underlying graph $\mathcal{G}$. Specifically, $G_t = (\mathcal{V}, E_t)$, where each edge $(i, j)$ in $\mathcal{G}$ appears in $E_t$ independently with probability $p$, i.e., $\mathbb{P}((i, j) \in E_t) = p.$
\end{assumption}


\begin{assumption}[Random Graph]
\label{ass: er_g}
    Assume that $\mathcal{G}$ is an arbitrary undirected connected graph. The communication network of the multi-agent system at time $t$ is modeled by a random graph $G_t$, which is generated over the underlying graph $\mathcal{G}$. Specifically, $G_t = (\mathcal{V}, E_t)$, where each edge $(i, j)$ in $\mathcal{G}$ appears in $E_t$ independently with probability $p$, i.e., $\mathbb{P}((i, j) \in E_t) = p.$
\hao{Hao will write more graph}

\begin{assumption}[Time-Dependent Networks] \Xu{$B$-Connected Graphs}
    
\end{assumption}

\begin{table}
    \centering
    \begin{tabular}{c|c|p{2cm}}
\cite{martinez2019decentralized} & $\sum_{k: \Delta_k>0} \frac{\ln (T N)}{\Delta_k}+(N \left\lceil\frac{\log (2 N )}{\sqrt{2 \ln \left(1 /\left|\lambda_2\right|\right)}}\right\rceil) \sum_{k=1}^K \Delta_k$  & homo and  fixed graph \\
\hline
\cite{zhu2021federated}
         &$\sum_{\Delta_k>0} \Delta_k\left(\max \left\{\frac{2 N^2}{\left(\frac{1}{2} \Delta_k-\alpha_1\right)^2} \log T, NL,(3 M+1) N^2\right\}+N\alpha_2\right)$  & hete fixed graph\\
\hline
\cite{xu2023decentralized}
         &\hao{MF can write here, too long. please multiply regret by N} & random graph p >1/2\\         
    \end{tabular}
    \caption{\hao{only for write good remarks} $\alpha_2=(3 M-1) N+\frac{2 \pi^2}{3}+\frac{2 \lambda_2^{1 / 12}}{\left(1-\lambda_2^{1 / 3}\right)\left(1-\lambda_2^{1 / 12}\right)} $
$L$ is the minimal value that satisfies $\lambda_2^{t / 6} /\left(1-\lambda_2^{1 / 3}\right)<(N t)^{-1}$}
    \label{tab:my_label}
    \title{}
\end{table}


\end{assumption}

==> secs/algortihm.tex <==
\section{Algorithm: \texttt{Gossip Successive Elimination}}
\label{sec: algorithms}
In this section, we present our proposed methodology. Unlike existing work on gossip bandits~\citep{martinez2019decentralized, zhu2021federated}, which assumes fixed connected graphs, we handle the fundamental challenges of randomness and possible disconnectivity in the random communication graph. To this end, we propose distributed bandit algorithm designed for Erdős–Rényi random graphs (\Cref{def: random_graph}) based on arm elimination, named \textit{Gossip Successive Elimination (GSE)} (\Cref{alg:GSE}). GSE combines three key components: an \textbf{arm elimination protocol}, a \textbf{refined weight matrix}, and a \textbf{novel confidence interval design}. Specifically, we adopt the arm elimination framework~\citep{even2006action} in distributed bandits setting, which naturally ensures that all agents pull each arm a comparable number of times, so that the global estimates obtained via gossip are not largely biased and not dominated by any single agent’s feedback. Second, we design a refined weight matrix based on the Laplacian, which guarantees that the weight matrices are i.i.d. across rounds. This construction is crucial to balance information among agents over time and to ensure that the global reward estimates converge to the true global mean reward for each arm. Finally, GSE introduces a new confidence interval with two terms: the first term captures the estimation error due to finite sampling, while the second term accounts for the consensus error, reflecting the approximation introduced by time-delayed information propagation under random gossip. Together, all these novel components enable GSE to jointly address reward heterogeneity and random communication in a principled and analytical paradigm.

The agent needs several parameters, including the link probability $p$ and algebraic connectivity $\lambda_{N-1}(\text{Lap}(\mathcal{G}))$ as inputs. Initially, agent $i$'s active arm set \(\mathcal{S}_i\) is set to the full set of arms \([K]\), while both the local reward estimate \(\muhat_{i,k}(t)\) and global reward estimate \(z_{i,k}(t+1)\) are initialized to zero ($t=0$). 
% Notably, Algorithm~\ref{alg:GSE} requires knowledge of the link probability \(p\) and the algebraic connectivity \(\lambda_{N-1}(\text{Lap}(\mathcal{G}))\).
Following the standard practice in existing work \citep{martinez2019decentralized, zhu2021federated,xu2023decentralized}, we assume that \(\lambda_{N-1}(\text{Lap}(\mathcal{G}))\) is known, while allowing the link probability \(p\) to remain unknown. In this case, the algorithm can still be implemented, and the corresponding regret upper bound preserved, by adding a short burn-in phase to estimate a value \(\hat{p} \in \left(\nicefrac{p}{2}, p\right]\). This estimation requires only \(\mathcal{O}(\log T)\) time steps. We refer the reader to Appendix~\ref{appendix: estimate_p} for the details and theoretical analysis of this procedure.

At each round \(t\), agent \(i\) observes its active neighbors \(\mathcal{N}_i(t)\) in the communication graph \(\mathcal{G}_t\), which is randomly generated from the base graph \({\mathcal{G}}\) according to \Cref{def: random_graph}. As part of our key contributions, we consider a weighting matrix \(W_t\) for gossip as
\begin{align}\label{align_calculation_of_W_t}
W_t = I_N - \frac{1}{N}\operatorname{Lap}(\mathcal{G}_t),
\end{align}
where \(\operatorname{Lap}(\mathcal{G}_t)\) denotes the Laplacian matrix of the communication graph \(\mathcal{G}_t\).
% Notably, the matrices \(W_t\) are independent and identically distributed, and $(\mathbb{E}[W_t W_t^\top]$ is symmetric and doubly stochastic. For simplicity, we denote \(\mathbb{E}[W^2] = \mathbb{E}_t[W_t W_t^\top]\). 

\begin{algorithm}[ht]
\caption{\texttt{Gossip Successive Elimination} for Agent \( i \in [N] \)}
\label{alg:GSE}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Algebraic connectivity \(\lambda_{N-1}(\textnormal{Lap}(\mathcal{G}))\), total time horizon \(T\), set of arms \([K]\), link probability $p$
\STATE {\bfseries Initialization:} Active set \(\mathcal{S}_i \leftarrow [K]\), local reward estimate \(\muhat_{i,k}(0) \leftarrow 0\), global reward estimate \(z_{i,k}(1) \leftarrow 0\) for all \(k \in [K]\).
\FOR{\(t = 1,2,\dots,T\)}
    \STATE Select arm \(A_i(t) \in \mathcal{S}_i\) with the minimum pull count \(T_{i,k}(t)\) and update $T_{i,k}(t)$
    \STATE Receive feedback and update statistics for each arm using \Cref{align_gossip_update}
    \STATE Remove arm \(k \in \mathcal{S}_i\) if there exists an arm \(k' \in \mathcal{S}_i\), \(k' \neq k\), satisfying the elimination condition in \Cref{align_elimination_rule}
    \STATE Update the active set \(\mathcal{S}_i\) according to \Cref{align_elimination_condition}
\ENDFOR
\end{algorithmic}
\end{algorithm}


The execution steps of agents run as follow. Agent $i$ selects arm \(A_i(t)\) from the active set \(\mathcal{S}_i\) with the least number of pulls \(T_{i,k}(t)\), observes the local reward of \(A_i(t)\), and updates the reward estimates as follows:
\begin{align}\label{align_gossip_update}
\muhat_{i,k}(t) &= \frac{1}{T_{i,k}(t) \vee 1}\sum_{\tau=1}^{t}\mathbb{I}\left\{ A_i(\tau)=k \right\} X_{i,k}(\tau), \notag \\
z_{i,k}(t+1) &= \sum_{j \in \mathcal{N}_i(t)\cup\{i\}} [W_t]_{i,j} z_{j,k}(t) + \muhat_{i,k}(t) - \muhat_{i,k}(t-1),
\end{align}
where \(X_{i,k}(\tau)\) is the feedback observed by agent \(i\) from pulling arm \(k\) at round $\tau$. The global estimate $z_{i,k}(t)$ is updated via a gossip protocol: at each round $t$, agent $i$ aggregates its own and its active neighbors’ estimates, weighting each neighbor $j\in\mathcal{N}_i(t)\cup\{i\}$ by the corresponding entry $[W_t]_{i,j}$ of the matrix $W_t$. We also define the gossip-based upper and lower confidence bounds for arm \(k\), which remain key criteria for arm elimination and updating \(\mathcal{S}_i\), as
\begin{align*}
\operatorname{GUCB}_{i,k}(t) = z_{i,k}(t) + c_{i,k}(t),\
\operatorname{GLCB}_{i,k}(t) = z_{i,k}(t) - c_{i,k}(t). 
\end{align*}
Here the confidence bound \(c_{i,k}(t)\) reads as 
\begin{align}\label{align_definition_of_c_ik(t)}
c_{i,k}(t) = \sqrt{\frac{4\log(T)}{N\max\{T_{i,k}(t)-KL^*,1\}}} + \frac{4(\sqrt{N}+\tau^*)}{\max\{T_{i,k}(t)-KL^*,1\}},
\end{align}
with
\begin{align}\label{align_definition_of_tau*_and_L}
\tau^* = \left\lceil \frac{2N\log(T)}{p\lambda_{N-1}(\textnormal{Lap}(\mathcal{G}))} \right\rceil,\ 
L^* = N\left\lceil -\frac{2\log(NT)}{\log(1-p)} \right\rceil.
\end{align}
The confidence radius in \Cref{align_definition_of_c_ik(t)} decomposes into two parts. The first term captures the \textbf{estimation error}, arising from the statistical variance of independently sampled rewards for each arm. The second term captures the \textbf{consensus error}, which stems from the cumulative approximation error error incurred as agents reach consensus via a gossip-based communication protocol.


Arm elimination occurs if and only if there exists an arm \(k' \neq k\) in \(\mathcal{S}_i\) that meets the condition
\begin{align}\label{align_elimination_rule}
\operatorname{GLCB}_{i,k'}(t) \geq \operatorname{GUCB}_{i,k}(t),
\end{align}
which means that arm $k'$ has a higher global reward estimate than arm $k$ with high probability. Subsequently, the active set \(\mathcal{S}_i\) is updated  as
\begin{align}\label{align_elimination_condition}
\mathcal{S}_i \leftarrow \bigcap_{j \in \mathcal{N}_i(t)\cup\{i\}} \mathcal{S}_j.
\end{align}

This procedure coupled with the arm‐elimination strategy ensures that, for every agent, each arm in the active set is pulled a roughly equal number of times, ensuring consensus.




==> secs/exps.tex <==
\section{Experiments}
\label{sec: exps}

In this section, we demonstrate the effectiveness of our algorithm through numerical experiments on both synthetic and real-world datasets.\footnote{The code for the experiments is available at \href{https://github.com/haoqiu95/multi-agent-bandit}{https://github.com/haoqiu95/multi-agent-bandit}.} The objective is twofold. First, we show that the cumulative regret of our algorithm grows logarithmically with respect to $T$ and is significantly smaller than that of existing benchmarks, thereby validating our theoretical findings. We use DrFed-UCB, proposed by \citep{xu2023decentralized}, as the baseline.  Second, we conduct a simulation study to examine how the regret depends on the link probability $p$ and the algebraic connectivity of the base graph $\mathcal{G}$, as reflected in the regret bound. We evaluate the impact of different values of $p$ across various base graphs, including the complete graph, grid, and Petersen graph \citep{holton1993petersen}. Each edge in the base graph $\mathcal{G}$ appears in the communication graph $\mathcal{G}_t$ with probability $p$. Moreover, we provide additional experiments (i.e., an ablation study) in \Cref{app: add_exps}, illustrating the regret dependency on the key parameters $p$ and $\lambda_{N-1}(\text{Lap}(\mathcal{G}))$ that determine the problem complexity beyond $T$, to validate our theoretical findings. %

\paragraph{Experimental Settings.}
For synthetic experiment setting, We set $T = 10000$, $N = 16$, and $K = 5$; for the Petersen graph, we use $N = 10$ by definition. For the comparison with DrFed-UCB, we consider a complete graph and a high link probability ($p = 0.9$), as required therein. Before the game starts, we sample each $q_i$ independently and uniformly from the interval $[0,1]$ for each agent $i$. The local mean reward of arm $k$ on agent $i$ is given by $\mu_{i,k} = q_i\cdot\frac{k-1}{K-1}$, and the global mean reward of arm $k$  is $\mu_k =\frac{k-1}{K-1}\cdot\frac{\sum_{i\in[N]}q_i}{N}$. At each time step $t$, each agent $i \in [N]$ selects an arm and observes the local reward. For real-world experiments, we use the MovieLens dataset and refer to \cite{yi2023doubly} for details. We set the horizon $T = 10{,}000$, and select 20 users as agents ($N = 20$) and 5 genres as arms ($K = 5$). At each time step $t$, each agent randomly selects a movie from the genres. All ratings (rewards) of movies are normalised to $[0,1]$.

\begin{figure*}[h]
    \centering
    \subfloat[Synthetic data]{%
        \includegraphics[width=0.43\textwidth]{new_neurips_2025/imgs/c_s-crop.pdf}%
        \label{fig:sc_dmax}
    }\hfill
    \subfloat[Real-world data]{%
        \includegraphics[width=0.43\textwidth]{new_neurips_2025/imgs/c_r-crop.pdf}%
        \label{fig:exp_dmax}
    }\hfill
    \subfloat[Synthetic data]{%
        \includegraphics[width=0.43\textwidth]{new_neurips_2025/imgs/vary_p_s-crop.pdf}%
        \label{fig:Syn_p}
    }\hfill
    \subfloat[Real-world data]{%
        \includegraphics[width=0.43\textwidth]{new_neurips_2025/imgs/vary_p_r-crop.pdf}%
        \label{fig:real_p}
    }
    \vspace{-2mm}
    \caption{Top two: comparison of the empirical results of our algorithm and DrFed-UCB (complete base graph, link probability $p=0.9$). Bottom two: regret of our algorithm on different base graphs as $p$ varies.} 
    \label{figure:compared}%
\end{figure*}

\paragraph{Experimental Results.}
All experiments are performed with $20$ independent replications. The shaded areas consider a range centered around the mean with half-width corresponding to the empirical standard deviation over $20$ repetitions. In \Cref{fig:sc_dmax,fig:exp_dmax}, we observe that our algorithm consistently outperforms DrFed-UCB on both synthetic and real-world datasets. In all runs, after an initial exploration period, our algorithm eliminates a significant number of suboptimal actions, resulting in near-constant regret thereafter. In \Cref{fig:Syn_p,fig:real_p}, we observe that increasing the link probability $p$ improves the algorithm’s performance, clearly validating the regret–communication trade-off. Additionally, different base graphs significantly impact the regret under the same $p$ value—with the complete graph yielding the lowest regret.

\section{Conclusion and Future Work}
\label{sec:conclusion}

In this paper, we study the multi-agent multi-armed bandit (MA-MAB) problem under general Erdős–Rényi random networks with heterogeneous rewards. To the best of our knowledge, we are the first to formulate MA-MAB with Erdős–Rényi random networks, where the communication graph is induced by a base graph and each edge in the base graph appears in the communication graph with probability $p$. This formulation generalizes the classical Erdős–Rényi model, in which the base graph is complete. We propose an algorithmic framework that incorporates the gossip communication protocol into arm elimination. Importantly, we analyze the regret bound of the algorithm and show that it improves the regret even under the classical Erdős–Rényi model. Moreover, our regret bound holds for any $p$, explicitly characterizes its dependency on $p$ and the algebraic connectivity of the base graph. This naturally reveals a trade-off between regret and communication efficiency. Moving forward, while we focus extensively on the stochastic setting, it would be valuable and exciting to explore other reward models—such as contextual bandits, where rewards depend on dynamic, non-stationary contexts. In addition, achieving the optimal trade-off among regret, communication, and privacy, as previously studied in homogeneous MA-MAB settings, points out a meaningful direction for future research.

\section*{Acknowledgments and Disclosure of Funding}
Jingyuan Liu and Lin Yang would like to thank the support from  NSFC (no. 62306138), JiangsuNSF (no. BK20230784), and the Innovation Program of State Key Laboratory for Novel Software Technology at Nanjing University (no. ZZKT2025B25). Hao Qiu acknowledges the financial support from the EU Horizon CL4-2022-HUMAN-02 research and innovation action under grant agreement 101120237, project ELIAS (European Lighthouse of AI for Sustainability) and from the One Health Action Hub, University Task Force for the resilience of territorial ecosystems, funded by Università degli Studi di Milano (PSR 2021-GSA-Linea 6).

==> secs/introduction.tex <==
\section{Introduction}\label{sec: Introduction} Multi-armed bandit (MAB) is a widely studied framework for sequential decision-making under uncertainty~\citep{ auer2002finite}. In this setting, an agent selects an arm from multiple options in each round, observes the reward from the chosen arm, and aims to maximize the cumulative expected reward. The emergence of large-scale cooperative systems holds true in various applications ranging from sensor networks~\citep{ganesan2004networking, zhu2016multi} to federated learning~\citep{ye2023heterogeneous, mcmahan2017communication} and edge computing~\citep{wang2022decentralized, ghoorchian2020multi}. It has naturally motivated interest in distributed multi-agent multi-armed bandit (MA-MAB) problem, where multiple agents collaboratively learn to optimize rewards. MA-MAB settings are typically categorized as homogeneous~\citep{landgren2016a, martinez2019decentralized} or heterogeneous~\citep{zhu2021federated, xu2023decentralized}, depending on whether the reward distributions for the same arm are identical across agents. The heterogeneous setting, in which reward distributions vary across agents, is significantly more general but more challenging, and thus has attracted growing attention. It introduces substantial difficulties, as agents must make sequential decisions under uncertainty while relying on limited information about both their own rewards and the actions or observations of other agents.

Another challenging aspect of MA-MAB lies in the underlying communication protocol, which constrains how agents share information with one another. Decentralized MA-MAB settings are more realistic than centralized ones—where all agents can communicate with any other agent—as they restrict communication to immediate neighbors defined by a graph structure. Much of the existing work has focused on time-invariant graphs~\citep{zhu2021federated}, where the communication graph remains fixed throughout. However, the complexity of many real-world decentralized systems, such as wireless ad-hoc networks, necessitates the use of time-varying graphs~\citep{zhu2023distributed}, particularly random graphs~\citep{xu2023decentralized}. This added complexity significantly complicates both the communication and learning dynamics. Notably, \citep{xu2023decentralized} is the first to consider classical Erdős–Rényi (E-R) random graphs in the MA-MAB setting, where any two agents can communicate with probability $p$ at each time step. However, it is possible that some pairs of agents can never communicate directly due to inherent topological constraints. This scenario has been formulated as a more general version of the E-R graph, where two agents can communicate with probability $p$ only if there is an edge between them in a base graph. Note that when the base graph is a complete graph, it is equivalent to classical (E-R) random graphs, implying consistency. To date, this setting remains unexplored, which motivates our work. 



To date, a line of work has studied regret bounds under various graph structures, where connectivity or sequential connectivity is typically required. For example, in the context of time-invariant graphs, \cite{martinez2019decentralized} and \cite{zhu2021federated} analyze distributed bandits over connected graphs and derive $\log T$ regret bounds. For time-varying graphs, \cite{zhu2025decentralized} obtains $\log T$ regret bounds under the assumption of B-connectivity, where the union of any $l$ consecutive graphs must be connected. In the classical Erdős–Rényi model \citep{erdos1960evolution} over fully connected agent communication, \cite{xu2023decentralized} derive a regret of order $\log T$ , but only under the assumption that $p \ge \nicefrac{1}{2} + \nicefrac{1}{2}\sqrt{1 - (\nicefrac{\epsilon}{NT})^{\nicefrac{2}{N-1}}}$ which is larger than $\nicefrac{1}{2}$ and can even approach 1 when the number of agents $N$ or the time horizon $T$ is large.  This is a strong assumption, as it may not hold in many real-world settings, but is required in their analysis to ensure that the graph is connected with high probability. Relaxing this connectivity requirement to allow arbitrary $p$ presents a significant challenge. Moreover, their regret bound does not reflect how the link probability $p$ impacts the regret. Incorporating $p$ into the regret expression would significantly improve our understanding of how to choose $p$ in practice—a gap that remains open. In this work, we address both of these gaps. To this end, we address the following key research question: \emph{Can we solve MA-MAB under new Erdős–Rényi random networks and heterogeneous rewards, and derive regret bounds that captures graph complexity under much milder assumptions?}


\paragraph{Contribution. }
We provide an affirmative answer to the above question via the following contributions. Methodologically, we solve the MA-MAB problem over general Erdős–Rényi communication networks with a gossip algorithm, which is widely adopted in distributed settings. Moreover, we adopt an arm elimination based algorithm with a minimal number of arm pulls required for each arm to guarantee sufficient information for each agent, which addresses the E-R communication networks. 

Analytically, we study the regret of MA-MAB under our proposed algorithm over general Erdős–Rényi communication networks for any $p \in (0, 1]$, leading to novel contributions. We are the first to 1) explore general Erdos-Rényi graphs induced by any fixed connected base graphs beyond classical setting that assumes a complete base graphs; 2) obtain a tighter and more interpretable regret bound, which generalizes the bound from the homogeneous fixed-graph setting studied in~\citet{martinez2019decentralized} to our more challenging heterogeneous setting, as shown in Section \ref{sec: theos}; 3) relax the assumption of a sufficiently large $p$ used in~\citet{xu2023decentralized} and reduce the order of $N$ in the upper bound in their analysis of classical Erdős–Rényi models with complete base graphs. Precisely, we obtain a regret upper bound of order of $\calO\left( \sum_{k:\Delta_k>0}\frac{\log T}{\Delta_k} + \frac{N^2\log T}{p\lambda_{N-1}(\text{Lap}(\mathcal{G}))}+\frac{KN^2\log T}{p} \right)$ where the first term accounts for an optimal centralized regret, aligning with the lower bound established in Section~\ref{sec: lower bound}, and the last two terms capture the effects of both the link probability $p$ and the algebraic connectivity $\lambda_{N-1}(\text{Lap}(\mathcal{G}))$ of the base graph. Moreover, we uniquely characterize how the regret upper bounds are influenced by $p$ and $\lambda_{N-1}(\text{Lap}(\mathcal{G}))$, which highlights a tradeoff between the communication cost (i.e., the number of communication rounds) and regret performance. 

Numerically, we implement our proposed algorithm and conduct experiments to validate our theoretical results with multiple random graph settings and the link probability $p$. We also compare our methods with existing approaches to demonstrate their effectiveness.

==> secs/related_work.tex <==
\section{Related Works}
\paragraph{Distributed online algorithm.} Our framework builds on the classical line of work on gossip algorithms \citep{xiao2004fast, boyd2006randomized}. Specifically, when an agent has access only to local information and communicates solely with its immediate neighbors, it adopts a gossip algorithm to aggregate information from agents beyond its local neighborhood, based on a weight matrix. 
Notably, gossip algorithms are widely used in distributed optimization. For example, \cite{duchi2011dual, nedic2009distributed} address distributed convex optimization problems using gossip algorithms. Subsequently, \cite{hosseini2013online,yan2012distributed} extend the gossip approach to the online setting and achieve a regret of order $\sqrt{T}$, assuming convex loss functions. Later, \cite{mateos2014distributed} consider distributed online optimization over B-connected and design a distributed online primal-dual algorithm coupled with a gossip protocol, also achieving a $\sqrt{T}$ regret bound. More recently, \cite{lei2020online} study the same problem over random communication networks (Erdős–Rényi networks) and obtain the same regret order. They further characterize how regret is affected by the link probability $p$ in the Erdős–Rényi model and the algebraic connectivity of the base graph $\mathcal{G}$. We consider the same graph topology but focus on multi-agent multi-armed bandits, which differ significantly from online convex optimization and introduce the additional challenge of learning the dynamics of bandits. For a more comprehensive survey on distributed online optimization, we recommend the reader to \citet{li2023survey} and \citet{yuan2024multi}.

\paragraph{Distributed multi-agent multi-armed bandit.} Along the line of work on MA-MAB, several studies \citep{landgren2016a, landgren2016b, zhu2020distributed, chawla2020gossiping, wangx2022achieving, wangp2020optimal, zhu2025decentralized, martinez2019decentralized, agarwal2022multi,sankararaman2019social,  zhu2021federated, zhu2023distributed, xu2023decentralized, yi2023doubly} have investigated both homogeneous and heterogeneous settings. In homogeneous settings, numerous works incorporate gossip algorithms to reduce regret in terms of the number of agents; information sharing among agents accelerates the concentration of reward observations. For example, \cite{landgren2016a, landgren2016b} firstly formulate this problem and solve it using gossip algorithms. \cite{martinez2019decentralized} achieves the optimal centralized regret—independent of the number of agents and matching that of the single-agent bandit—plus an additional term depending on the spectral gap of the communication matrix. \citet{chawla2020gossiping} characterizes the regret-communication tradeoff, considers circular ring graphs, and improves regret. \cite{wangx2022achieving, wangp2020optimal} further focus on optimizing communication efficiency to minimize the number of communication rounds while guaranteeing regret performance. In contrast, we consider more challenging heterogeneous settings and also characterize the regret-communication trade-off. Here gossiping enables regret reduction in terms of the order of $T$; without information from other agents, the regret can easily be linear in $T$ \citep{xu2025multi}. In this direction, \cite{zhu2021federated} is the first to study heterogeneous rewards over a time-invariant connected graph and establishes regret bounds of order $\log T$. \citet{zhu2023distributed} extend this to B-connected graphs, also achieving regret bounds of order $\log T$. Recently, \cite{xu2023decentralized} propose a gossip-based algorithm for the classical E-R model and obtain regret bounds of order $\log T$ when $p$ is sufficiently larger than $1/2$ to ensure the graph is connected with high probability. More generally, \cite{yi2023doubly} consider MA-MAB with heterogeneous rewards in the adversarial environment and establishes a regret bound of order $T^{2/3}$. In contrast, we consider the stochastic setting with general Erdős–Rényi random networks, without any assumption on $p$.
  

==> secs/setting.tex <==
\section{Setting and Notations}
\label{sec:setting}
In this section, we formally define the problem of interest, starting with general notations. A full notation chart can be found in \Cref{appendix: notation}.

\paragraph{General Notations.} For a matrix $M \in \mathbb{R}^{p \times q}$, let $[M]_{i, j}$ denote the entry in the $i$-th row and $j$-th column. Given a doubly stochastic matrix $P \in \mathbb{R}^{d \times d}$, we denote by $\lambda_2(P)$ its second largest eigenvalue. Let $e_i \in \mathbb{R}^d$ be the $i$-th standard basis vector, $\mathbf{1} \in \mathbb{R}^d$ the all-ones vector, and $I_d$ the $d \times d$ identity matrix. We use $\Ind{\cdot}$ to denote the indicator function, which equals $1$ if the condition inside holds, and $0$ otherwise. Moreover, we use $[n]=\{1,2,\cdots,n\}$ to denote a set of indices.


\paragraph{Multi-Agent Multi-armed Bandit.} We consider a multi-agent multi-armed bandit (MA-MAB) setting involving $N$ agents. The bandit problem is run over a time horizon of $T$.

In each round $t \in [T]$, every agent $i \in [N]$ selects an arm $A_i(t) \in [K]$ and receives a local stochastic reward $X_{i,A_i(t)}(t)$ drawn independently from an unknown, time-invariant distribution $\mathbb{P}_{i,A_i(t)}$ supported on $[0,1]$, with mean $\mu_{i,A_i(t)} = \mathbb{E}[X \sim \mathbb{P}_{i,A_i(t)}] \in [0,1]$.
However, the agent's true objective depends on the global reward $X_{A_i(t)}(t)$, where $X_{A_i(t)}\coloneqq\frac{1}{N}\sum_{j\in[N]}X_{j,A_i(t)}(t)$, which is the average reward over all agents and is not observable by any agent. Accordingly, we define the global mean reward for arm $k$ as $\mu_k\coloneqq\frac{1}{N}\sum_{j\in[N]}\mu_{j,k}$ by taking the expectation of $X_{k}(t)$, where $\mu_{j,k}$ is the mean of $\mathbb{P}_{j,k}$. The underlying target is to optimize the global mean reward, and hence agents require estimates of the global mean reward values for each arm in order to identify the global optimal arm with the highest global mean reward. 
We further use $T_{i,k}(t)$ to denote the total number of times agent $i$ has selected arm $k$ up to time $t$ by $T_{i,k}(t) = \sum_{s=1}^t \mathbb{I}(A_i(s) = k)$.


Throughout, we focus on a decentralized setting where $N$ agents are distributed on undirected time-varying graphs and communicate via the graphs. Specifically, we consider a communication graph based on \textit{Erdős–Rényi random graphs}. More precisely, agents communicate via a time-varying graph $\mathcal{G}_t = (\mathcal{V}, \mathcal{E}_t)$, where the vertex set $\mathcal{V} = [N]$ is fixed, but the edge set $\mathcal{E}_t$ may vary at each round $t$. Uniquely, each \textit{communication graph} $\mathcal{G}_t$ is generated based on an underlying undirected, fixed, and connected (but not necessarily complete) \textit{base graph} ${\mathcal{G}} = (\mathcal{V}, {\mathcal{E}})$ that defines all feasible communication edges. The connectedness of the base graph is essential to avoid linear regret as proved in Theorem 4 in~\citet{xu2025multi}. In every round $t$, each edge in graph ${\mathcal{G}}$ is independently in $\mathcal{G}_t$ with probability $p \in (0,1]$. Two agents can communicate if and only if there is an edge between them in $\mathcal{G}_t$—namely, an active edge. Formally, the random graph generation reads as follows.
\begin{assumption}[Erdős–Rényi Random Graph]
\label{def: random_graph}
In each round $t$, the random communication graph $\mathcal{G}_t = (\mathcal{V}, \mathcal{E}_t)$, generated from the base graph $\mathcal{G}$ meets:
\begin{align*}
\mathbb{P}\left((i,j) \in \mathcal{E}_t\right)=
\begin{cases}
p, & \text{if } (i,j) \in \mathcal{E}, \\
0, & \text{otherwise,}
\end{cases}
\end{align*}
for all vertices \( i,j \in \mathcal{V} \). We refer to $p$ as the \textit{link probability}.
\end{assumption}
Thus, \( \mathcal{E}_t \subseteq {\mathcal{E}} \) for all \( t \). Let \( \mathcal{N}_i = \{j \in \mathcal{V} : (i,j) \in {\mathcal{E}}\} \) denote the neighbors of agent \( i \) in the base graph \( {\mathcal{G}} \), and \( \mathcal{N}_i(t) = \{j \in \mathcal{V} : (i,j) \in \mathcal{E}_t\} \) denote the active neighbors of agent \( i \) in round \( t \), clearly satisfying \( \mathcal{N}_i(t) \subseteq \mathcal{N}_i \). 

The shared objective for each agent is to design a distributed algorithm $\pi$ that minimizes the global regret over $T$ rounds; in other words, all agents share a common target that makes consensus possible and necessary. Precisely, we first define the individual regret, which represents the objective of any agent $i\in[N]$, as:
\begin{align}\label{a1}
\textnormal{Reg}_{i,T}(\pi) = T\mu^* - \sum_{t=1}^T\mu_{A_i(t)} = \sum_{t=1}^T\Delta_{A_i(t)},
\end{align}
where $\mu^*=\max_{k\in[K]}\mu_k$ is the optimal global mean reward, and $\Delta_k=\mu^*-\mu_k$ is the global suboptimality gap for arm $k$. Notably, agents aim to optimize the global mean rewards of the pulled arms, i.e., to pull the global optimal arm. We define the individual regret as the cumulative difference between the global mean reward of the global optimal arm and that of the actual arm pulled by each agent. Building on this, we define the global regret of the entire system for algorithm $\pi$ as the sum of the individual regret over all agents:
\begin{align}\label{a2}
\textnormal{Reg}_T(\pi) = \sum_{i\in[N]}\textnormal{Reg}_{i,T}(\pi) = NT\mu^* - \sum_{i\in[N]}\sum_{t=1}^T\mu_{A_i(t)} = \sum_{i\in[N]}\sum_{t=1}^T\Delta_{A_i(t)},
\end{align}
which establishes the equivalence of \Cref{a1} in the context of individual agents.


==> secs/theoretical_results.tex <==
\section{Regret Analyses} \label{sec: theos}

In this section, we analyze the regret of the proposed algorithm and establish an upper bound on the corresponding regret, demonstrating its theoretical effectiveness. Additionally, we derive a lower bound for our problem setting, highlighting the problem’s inherent complexity and showing that the algorithm is nearly optimal up to some interpretable factors.


\subsection{Upper Bound}
We start by presenting the regret upper bound for \Cref{alg:GSE}. To that end, we first introduce several technical lemmas that play a key role in the regret analysis. The proofs can be found in \cref{appendix: theorem}.

\begin{lemma}
\label{theorem: upperbound}
\label{confidence_bound}
Let us assume that the communication graph follows \Cref{def: random_graph}. Then we have that for \Cref{alg:GSE}, for any agent $i \in [N]$, any arm $k \in [K]$, and any $t \in [T]$, the following holds with probability at least $1 - \frac{3NK}{T}$, 
\begin{align*}
|z_{i,k}(t) - \mu_k| \leq c_{i,k}(t),
\end{align*}
where $c_{i,k}(t)$ is the confidence bound defined in \Cref{align_definition_of_c_ik(t)}, and $\tau^*$ and $L^*$ are the parameters introduced in \Cref{align_definition_of_tau*_and_L}.
\end{lemma}

Importantly, we show that the estimation error compared to the global mean value is upper bounded by the confidence bound $c_{i,k}(t)$. Notably, $c_{i,k}(t)$ is monotonically decreasing in the number of pulls of arm $k$ by agent $i$, i.e., $T_{i,k}(t)$, when $T_{i,k}(t) > KL^*$. Here, $KL^*$ is the minimal number of pulls required to ensure that agent $i$ has collected sufficient information from all other agents. This also implies that the global estimate $z_{i,k}(t)$ becomes increasingly accurate and approaches the true mean reward $\mu_k$ as the number of pulls increases. As a result, based on \Cref{confidence_bound}, we derive the following regret bound for individual agents.

\begin{lemma}\label{align_regret_for_single_arm}
Let us assume that the communication graph follows \Cref{def: random_graph}. The individual regret of agent $i$ defined in \Cref{a1} for \Cref{alg:GSE} is bounded as:
\begin{align*}
\textnormal{Reg}_{i,T}(\textnormal{GSE}) \leq \sum_{k: \Delta_k>0} \left( \frac{64 \log(T)}{N \Delta_k} + 16\left(\sqrt{N} + \tau^*\right) \right) + KL^* + 3KN \Delta_{\max},
\end{align*}
where $\Delta_{\max} = \max_{k \in [K]} \Delta_k$ denotes the largest reward gap across all arms. 
\end{lemma}

In other words, \Cref{align_regret_for_single_arm} shows that the regret incurred by any individual agent can be effectively bounded. This result naturally extends to the global regret, as stated in the theorem below.
\begin{theorem}\label{th1}
Let us assume that the communication graph follows \Cref{def: random_graph}. The global regret defined in \Cref{a2} for \Cref{alg:GSE} is bounded as:
\begin{align*}
\textnormal{Reg}_T(\textnormal{GSE})=\sum_{i\in[N]}\textnormal{Reg}_{i,T}(\textnormal{GSE}) 
&\leq \calO\left(\sum_{k: \Delta_k>0} \frac{\log(T)}{\Delta_k} + \frac{N^2\log(T)}{p \lambda_{N-1}(\operatorname{Lap}(\calG))} + \frac{KN^2 \log(NT)}{p} \right),
\end{align*}
where $\lambda_{N-1}(\operatorname{Lap}(\calG))$ is the second smallest eigenvalue of $\operatorname{Lap}(\calG)$.  
\end{theorem} 

We continue our discussion on how the base graph ${\calG}$ topology affects the regret bound. In addition to the parameter $p$, which determines the difference between ${\calG}$ and $\calG_t$, another key factor is $\lambda_{N-1}(\operatorname{Lap}(\calG))$, which reflects the topology of the base graph ${\calG}$. This value is the algebraic connectivity or Fiedler value of $\calG$, which reflects how well connected the overall graph is.  To illustrate this, we next provide more explicit regret upper bounds by specifying $\lambda_{N-1}(\operatorname{Lap}(\calG))$ for different base graph topologies commonly used in distributed optimization \cite{duchi2011dual}. The following corollary summarises how the choice of the random gossip matrix in \cref{align_calculation_of_W_t} interacts with different topologies of the base graph. The proof of $\lambda_{N-1}(\operatorname{Lap}(\mathcal{G}))$ for various base graphs $\mathcal{G}$ can be found in Corollary~1 of \cite{duchi2011dual}.

\begin{corollary}\label{coro: topology}
For specific choices of the base graph \(\mathcal{G}\), the global regret upper bound in \Cref{th1} simplifies as follows:

1) When \(\mathcal{G}\) is a complete graph with \(\lambda_{N-1}(\operatorname{Lap}(\mathcal{G})) = N\), and refining \(L^* = \left\lceil -\frac{2 \log(NT)}{\log(1 - p)} \right\rceil\) in \Cref{align_definition_of_tau*_and_L}, \Cref{th1}
simplifies to:
\(
\mathcal{O}\left( \sum_{k : \Delta_k > 0} \frac{\log T}{\Delta_k} + \frac{KN \log T}{p} \right).
\)

2) When \(\mathcal{G}\) is a \(\sqrt{N} \times \sqrt{N}\) 2D grid with \(\lambda_{N-1}(\operatorname{Lap}(\mathcal{G})) = 2\left(1 - \cos\left( \frac{\pi}{\sqrt{N}} \right)\right) = \Theta(1/N)\), \Cref{th1} simplifies to:
\(
\mathcal{O}\left( \sum_{k : \Delta_k > 0} \frac{\log T}{\Delta_k} + \frac{N^2\left(K + N\right) \log T}{p} \right).
\)

3) When \(\mathcal{G}\) is an expander graph with a bounded ratio between minimum and maximum node degrees and thus \(\lambda_{N-1}(\operatorname{Lap}(\mathcal{G})) = \Theta(1)\), \Cref{th1} simplifies to:
\(
\mathcal{O}\left( \sum_{k : \Delta_k > 0} \frac{\log T}{\Delta_k} + \frac{KN^2 \log T}{p} \right).
\)

\end{corollary}



\begin{remark}[Comparison of Regret Bounds] 
In \cref{th1}, for any fixed connected base graph $\mathcal{G}$ and $0 < p \leq 1$, we obtain the optimal centralized regret $\calO\left( \sum_{k:\Delta_k>0}\frac{\log T}{\Delta_k} \right)$ (see the lower bound in \Cref{sec: lower bound}) plus an additional term $\calO\left(\frac{N^2 \log T}{p \lambda_{N-1}(\operatorname{Lap}(\calG))} + \frac{KN^2 \log T}{p}\right)$. We emphasize that our regret bound outperforms existing work—many of which are special (degenerated) cases of our more general framework—and is easier to interpret. Notably, \cite{xu2023decentralized} study MA-MAB under the classical E-R model (where $\mathcal{G}$ is a complete graph) with $p$ largely over $1/2$, and derive a regret bound of $\mathcal{O}\left(\sum_{k:\Delta_k > 0} \frac{N\log T}{\Delta_k}\right)$. In the same setting, based on \Cref{coro: topology}, we obtain a regret bound of $\calO\left(\sum_{k: \Delta_k > 0} \frac{\log(T)}{\Delta_k}  + KN\log(T) \right)$, which is significantly smaller. Also, \cite{zhu2023distributed} consider B-connected graphs, which do not capture E-R random graphs; the distinction between the two models is discussed in detail in \cite{yuan2024multi}. Finally, when $p = 1$, the communication graph becomes time-invariant, which corresponds to most existing work where connected graphs are assumed. For example, \cite{zhu2021federated} and \cite{zhu2023distributed} study such settings. The former derive a regret bound of $\mathcal{O}\left(\sum_{k: \Delta_k > 0} \frac{N^2\log T}{\Delta_k}\right)$, which is worse than our results with a dependency on $N$. The latter obtain $ \mathcal{O}\left(\max\left(\sum_{k: \Delta_k > 0} \frac{N\log T}{\mathcal{N}_k\Delta_k}, K_1, K_2\right)\right)$, where $K_1$ and $K_2$ depend on $T$ but lack explicit formulas, may grow arbitrarily large, and are difficult to interpret—at least to the best of our knowledge. 

\end{remark}


\begin{remark}[Regret and Communication Trade-off]
    We emphasize that our regret upper bound exhibits a novel trade-off between regret performance and communication efficiency in the presence of random graphs. It is straightforward to observe that increasing $p$ reduces the regret bound but increases communication overhead, thereby lowering communication efficiency. For classical E-R graphs, the expected number of agent-to-agent communications per agent over the given time horizon is $p N T$, while the expected regrets decrease as $p$ increases.  Therefore, for a fixed time horizon $T$ and a given base graph ${\mathcal{G}}$, $p$ can be tuned to balance communication overhead and reward maximization, informing practical decision making. 
\end{remark}




\subsection{Lower Bound}\label{sec: lower bound}
In this section, we establish a lower bound on the global regret, as defined in \Cref{a2}. Unlike the upper bound, this lower bound applies to any reasonable algorithm under a specific problem instance, highlighting the problem complexity.  Detailed proofs are deferred to Appendix \ref{appendix: theorem}. We begin by introducing several definitions related to the problem instance and the notion of a reasonable algorithm.

\begin{definition}[Gaussian Instance]
An instance $\nu$ is called a \emph{Gaussian instance} if, for every agent $i \in [N]$ and arm $k \in [K]$, the reward distribution $\mathbb{P}_{i,k}$ is Gaussian with unit variance.
\end{definition}

\begin{definition}[Consistent Policy]
Let $\mathcal{I}$ denote a class of problem instances, and let $\text{Reg}_T^{\nu}(\pi)$ denote the regret incurred by policy $\pi$ on instance $\nu$. A policy (algorithm) $\pi$ is said to be \emph{consistent} on $\mathcal{I}$ if there exist constants $C > 0$ and $s \in (0,1)$ such that $\text{Reg}_T^{\nu}(\pi)$ meets $
\text{Reg}_T^{\nu}(\pi) \leq C T^s$
for all instances $\nu \in \mathcal{I}$. 
\end{definition}

We next present the problem instance constructed to establish the regret lower bound. Note that an alternative, equivalent expression of the global regret reads as 
\[
\text{Reg}_T^{\nu}(\pi) = \sum_{k \in [K]} \Delta_k \sum_{i \in [N]} \mathbb{E}[T_{i,k}(T)].
\]
Thus, to derive a lower bound on regret, it suffices to lower bound the total expected number of pulls $\sum_{i \in [N]} \mathbb{E}[T_{i,k}(T)]$ for  suboptimal arms $k \in [K]$. To this end, we consider a Gaussian instance $\nu$ where each $\mathbb{P}_{i,k} = \mathcal{N}(\mu_{i,k}, 1)$ with the random graph communication protocal based any connected base graph $\mathcal{G}$ and connection probability $p$, and construct a perturbed instance $\nu'$ such that:
\[
\mathbb{P}'_{i,a} =
\begin{cases}
\mathcal{N}(\mu_{i,a}, 1), & \text{if } a \neq k, \\
\mathcal{N}(\mu_{i,a} + (1+\varepsilon)\Delta_a, 1), & \text{if } a = k,
\end{cases}
\]
for a small constant $\varepsilon \in (0,1)$ representing the level of perturbation. The communication protocal for $\nu'$ is the same as that for $\nu$. Under this perturbation, which defines a new problem instance, we derive the following information-theoretic inequality: 
\begin{align}\label{align_lower_bound_for_total_pulling_rounds}
\sum_{j \in [N]} \mathbb{E}[T_{j,k}(T)] \cdot \frac{(1+\varepsilon)^2 \Delta_k^2}{2} \geq \log\left( \frac{NT \varepsilon \Delta_k}{4\left(\text{Reg}_T^{\nu}(\pi) + \text{Reg}_T^{\nu'}(\pi)\right)} \right),
\end{align}
which imposes a lower bound on the total number of pulls of arm $k$ across all agents.

By applying this inequality to a consistent policy $\pi$ and rearranging the terms, we obtain the following lower bound on regret. The formal statement reads as follows. 

\begin{restatable}{theorem}{lowerbound}
\label{theorem: lowerbound}
Let $\pi$ be a consistent policy on the class $\mathcal{I}$ of Gaussian instances for some $s \in (0,1)$. Then, for all instances $\nu \in \mathcal{I}$ and any $\varepsilon \in (0,1]$, the following holds:
\[
\lim_{T \rightarrow \infty} \frac{\textnormal{Reg}_T^{\nu}(\pi)}{\log T} \geq \sum_{k: \Delta_k>0} \frac{2(1-s)}{(1+\varepsilon)^2 \Delta_k}.
\]
\end{restatable}

\begin{remark}[Comparison with Upper Bounds]
Recall that the regret upper bound in \Cref{th1} consists of two terms: a centralized term and additional terms that capture the influence of the communication graph. The lower bound in \Cref{theorem: lowerbound} shows that the centralized component, \(\mathcal{O}\left( \sum_{k:\Delta_k>0}\frac{\log T}{\Delta_k} \right)\), is tight, thereby establishing the optimality of the centralized regret achieved by Algorithm~\ref{alg:GSE}. This result is intuitive: the problem effectively involves \(N\) agents collaboratively solving a global multi-armed bandit task. With appropriate information sharing, the collective performance can match that of a single-agent bandit problem with full access to all rewards. Hence, achieving a global regret of the same order as the classical centralized bandit setting is both natural and optimal. The additional term related to the communication graph, though not captured in \Cref{theorem: lowerbound}, can be interpreted intuitively. Consider, for instance, a circular base graph $\mathcal{G}$: on average, it takes $O(N/p)$ rounds for information from one agent to propagate to all others. Aggregating over all $N$ agents, this leads to an unavoidable lower bound of $O(N^2/p)$ in the global regret. Providing a formal lower bound proof that fully characterizes this effect remains an interesting direction for future work.
\end{remark}


